Popular Matching in Roommates Setting is NP-hard

An input to the Popular Matching problem, in the roommates setting, consists of a graph $G$ and each vertex ranks its neighbors in strict order, known as its preference. In the Popular Matching problem the objective is to test whether there exists a matching $M^\star$ such that there is no matching $M$ where more people are happier with $M$ than with $M^\star$. In this paper we settle the computational complexity of the Popular Matching problem in the roommates setting by showing that the problem is NP-complete. Thus, we resolve an open question that has been repeatedly, explicitly asked over the last decade.

==> introOLD.tex <==
% !TEX root = mainPM.tex

\newcommand{\Ma}[1]{\textcolor{magenta}{#1}}
\newcommand{\ma}[1]{\todo[line, color={Yellow}]{\footnotesize{#1}}\xspace}
\newcommand{\il}[1]{\todo[inline, color={Yellow}]{{#1}}}
\newcommand{\etalcite}[1]{\emph{et~al.}~\cite{#1}}
\newcommand{\etal}{\emph{et~al.}\xspace}


\section{Introduction}\label{sec:intro}

%\hly{TODO}

%\ma{Problem Def}
The input to the \popular\ problem consists of a graph on $n$ vertices and the preferences of the vertices represented as a ranked list of the neighbors of every vertex, said to be the {\it preference list} of the vertex. The goal is to find a {\it popular matching}--a matching that is preferred over any other matching (in terms of the preference lists) by at least half of the vertices in the graph. 

\popular\ is one of the best known problems in the topic {\it matchings under preferences}, a class of matching problems that requires that the matching obtained satisfy some predefined notion of acceptability of the participating vertices. It is well-known that when the input graph is bipartite, \popular\ problem can always be decided affirmatively in polynomial time, \cite{DBLP:journals/iandc/HuangK13}. It is equally well-known that when the graph is arbitrary, the computational complexity of deciding whether a popular matching exists is unknown. In this paper we settle this question by proving the following result. 
\begin{theorem}\label{thm:main}
\popular\ is \NPH.
\end{theorem}

%\ma{Appl of PM}
Popular matching finds real-life applications in avenues as diverse as the organ-donor exchange markets, spectrum sharing in cellular networks, barter exchanges, to just name a few \cite{XiaoHanYuenDaSilva16}. Specifically, situations in which a {\it stable matching} -- a matching that does not admit an edge whose endpoints prefer each other to their respective ``situation'' in the current matching -- is too restrictive, popular matching finds applicability. It is known that stable matching is the smallest sized popular matching. So for applications where it is desirable to have matchings of size larger than a stable matching -- for instance, allocating projects to students,
where the absence of blocking edges is not mandatory -- popular matching may be a suitable alternative.The notion of popularity captures a natural relaxation of the notion of stability: blocking edges are permitted but the matching, nevertheless has overall stability. 

%\ma{History}
The provenance of the notion of a popular matching can be dated to the work of Condorcet in 1785 on the subject of a {\it Condorcet winner} \cite{Condorcet1785}. In the last century, however, the notion was introduced as the {\it majority assignment} by G\"{a}rdenfors \cite{Gardenfors75} in 1975. Anecdotal retelling ascribes the coinage of the term ``popular matching'' and the associated question of does there exist a polynomial time algorithm for \popular\ to Robert Irving during a talk in University of Glasgow in 2012, \cite[pg 303]{Manlove13b}. Abraham \etalcite{Abraham07} was the first to discuss an efficient algorithm for computing a popular matching albeit for the case where the graph is bipartite and only the vertices in one of the partitions have a preference list, an setting known as the {\sf Housing Allocation}. The persuasive motivation and elegant analysis of Abraham \etal led to a spate of papers on popular matching \cite{ManloveSng06,HuangKavithaMichailNasre08,KavithaN09,KavithaMestreNasre11,OptimalPM09,BiroIrvingManlove10,HuangKavitha17,KiralyKarkus17} covering diverse settings that include strict preferences as well as one with ties. %\ma{Huang,Manlove}


In the midst of this work, the issue of the computational complexity of \popular\ in an arbitrary graph remained unsettled, leading various researcher to devise notions such as the {\it unpopularity factor} and {\it unpopularity margin} \cite{HuangKavithaMichailNasre08,McCutchen08,HuangKavitha13j} in the hope of capturing the essence of popular matchings. A solution concept that emerged from this search is the {\it maximum sized popular matching}, motivated by the fact that unlike stable matchings (Rural Hospital Theorem \cite{Roth86}), all popular matchings in an instance do not match the same set of vertices or even have the same size. Thus, it is natural to focus on the size of a popular matching. There is a series of papers that focus on computing the maximum sized popular matchings in bipartite graphs (without ties in preference lists) \cite{Size-Popularity-Tradeoff-Kavitha14j,DBLP:journals/iandc/HuangK13,CsehKavitha16} and (with ties) \cite{PM-2sidedPref-1sidedTies-CsehHuangKavitha17j}. When preferences are strict, there are various polynomial time algorithm that compute a maximum sized popular matching in bipartite graphs: Huang and Kavitha \cite{HuangKavitha13j} give an $\mathcal{O}(mn_{0})$ algorithm that is improved by Kavitha to $\mathcal{O}(m)$ \cite{Size-Popularity-Tradeoff-Kavitha14j} where $m$ and $n_{0}$ denote the number of edges in the bipartite graph and the size of the smaller vertex partition, respectively. In the presence of ties (even on one side), the problem of computing the maximum sized popular matching was shown to be \NPH\ \cite{PM-2sidedPref-1sidedTies-CsehHuangKavitha17j}. It is worth noting that every stable matching is popular, but the converse is not true. As a consequence of the former, every bipartite graph has a popular matching that is computable in polynomial-time because it has a stable matching computable by the famous Gale-Shapley algorithm described in the seminal paper \cite{GaleShapley62} by the eponymous Gale and Shapley. Recently, Kavitha investigated the computational complexity of the search for a maximum sized popular matching in arbitrary graphs \cite{DBLP:journals/corr/abs-1802-07440}, and showed it to be \NPH.

%\ma{terminology}
In literature, the terminology related to \popular\ is closely related to that of the {\sc Stable Marriage} problem. 
When the input graph is (bipartite) arbitrary, the instance is said to be that of the ({\sc Stable Marriage}) {\sc Stable Roommate} problem. 









==> preamble.tex <==
\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

%for urls
\usepackage{url}

\usepackage[dvipsnames,svgnames,x11names]{xcolor}

\usepackage{soul}

\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}
%

\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
%\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}

\usepackage{graphics}
\usepackage{pgf}
\usepackage{paralist} 
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
%\usepackage{todonotes}

\newcommand{\OO}{\mathcal{O}}

\usepackage{vmargin}
\setmarginsrb{1in}{1in}{1in}{1in}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{definition}{Definition}[section]
\newtheorem{observation}{Observation}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{redrule}{Reduction Rule}[section]
\newtheorem{remark}{Remark}[section]
\newtheorem{reduction}{Reduction Rule}[section]
\newtheorem{conjecture}{Conjecture}[section]

\date{}
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

% general
\newcommand{\yes}{\textsf{Yes}}
\newcommand{\no}{\textsf{No}}
\newcommand{\yesinstance}{\yes-instance}
\newcommand{\noinstance}{\no-instance}
\newcommand{\tw}{\mathtt{tw}}
\newcommand{\NP}{\textsf{NP}}
\newcommand{\coNP}{\textsf{co-NP}}
\newcommand{\FPT}{\textsf{FPT}}
\newcommand{\XP}{\text{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}

% specific
\newcommand{\popular}{{\sc Popular Matching}}
\newcommand{\pvc}{{\sc Partitioned Vertex Cover}}
\newcommand{\vote}{\mathtt{vote}}
\newcommand{\red}{\mathtt{reduction}}
\newcommand{\lab}{\mathtt{label}}

\usepackage{booktabs}

\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref} 

\usepackage{tikz}
\usepackage{xkeyval}
%\usepackage[textsize=small,obeyDraft]{todonotes}
\usepackage[textsize=small]{todonotes}



